A Multi-Power Law for Loss Curve Prediction Across Learning Rate Schedules

Training large models is both resource-intensive and time-consuming, making it crucial to understand the quantitative relationship between model performance and hyperparameters. In this paper, we present an empirical law that describes how the pretraining loss of large language models evolves under different learning rate schedules, such as constant, cosine, and step decay schedules. Our proposed law takes a multi-power form, combining a power law based on the sum of learning rates and additional power laws to account for a loss reduction effect induced by learning rate decay. We extensively validate this law on various model sizes and architectures, and demonstrate that after fitting on a few learning rate schedules, the law accurately predicts the loss curves for unseen schedules of different shapes and horizons. Moreover, by minimizing the predicted final pretraining loss across learning rate schedules, we are able to find a schedule that outperforms the widely used cosine learning rate schedule. Interestingly, this automatically discovered schedule bears some resemblance to the recently proposed Warmup-Stable-Decay (WSD) schedule (Hu et al, 2024) but achieves a slightly lower final loss. We believe these results could offer valuable insights for understanding the dynamics of pretraining and designing learning rate schedules to improve efficiency.

==> main/derivations/bottomup2.tex <==
\subsection{Bottom-Up Derivation: Two-Stage, Multi-Stage, and General Schedules}\label{sec:bottom-up}

The challenges in approximating the intermediate loss reduction $\LD_k(t)$ are twofold. First, for commonly used schedules, the learning rate (LR) reduction at intermediate steps is often too small to induce a measurable loss reduction. Second, $\LD_k(t)$ may depend intricately on all previous learning rates $\{\eta_1, \dots, \eta_{k}\}$, which we refer to as the \textit{LR prefix} in this section. To address these issues, we derive the form of $\LD_k(t)$ using a ``bottom-up" approach regarding schedule structures. Initially, we propose its form through schedules comprising two constant LR stages, leveraging significant LR reductions. Next, we examine its dependency on the LR prefix using schedules of multiple stages. Finally, we generalize the form to encompass all schedules and conclude with our multi-power law.

\subsubsection{Case 1: Two-Stage Learning Rate Schedule}\label{section two-stage}\label{sec:two-stage}
\input{main/derivations/two_stage}
\subsubsection{Case 2: Multi-Stage Learning Rate Schedule} \label{sec:multi-stage}
\input{main/derivations/multi_stage}
\subsubsection{Case 3: General Learning Rate Schedule}\label{section general lrs}

\input{main/derivations/general}

==> main/derivations/bottomup3.tex <==
\subsection{Bottom-Up Derivation: Two-Stage, Multi-Stage, and General Schedules}\label{sec:bottom-up}

The challenges in approximating the intermediate loss reduction $\LD_k(t)$ are twofold. First, for commonly used schedules, the learning rate (LR) reduction at intermediate steps is often too small to induce a measurable loss reduction. Second, $\LD_k(t)$ may depend intricately on all previous learning rates $\{\eta_1, \dots, \eta_{k}\}$, which we refer to as the \textit{LR prefix} in this section.

To address these issues, we derive the form of $\LD_k(t)$ using a ``bottom-up" approach regarding schedule structures. First, we propose its form through schedules comprising two constant LR stages, leveraging significant LR reductions. Next, we examine its dependency on the LR prefix using schedules of multiple stages.
Our main finding is that $\LD_k(t)$ depends weakly on the LR prefix and can be approximated by the following form:
\begin{align}\label{eq:prefix-independent}
\LD_k(t)\approx\hatLD_k(t):=B (\eta_{k} - \eta_{k+1}) \left(1-\left(C\eta_{k+1}^{1-\gamma}(t-k)+1\right)^{-\beta}\right),
\end{align}
with LR-prefix independent constants $B$, $C$, $\gamma$ and $\beta$.
Due to space constraints, we refer readers to~\Cref{sec:two-stage,sec:multi-stage} for detailed derivations of~\eqref{eq:prefix-independent}.


\begin{figure}[t!]
\vspace{-0.4in}
    \centering
    \subfigure[Cyclic Schedule]{
    \includegraphics[width=0.48\linewidth]{figures/25M/cyclic_72000.pdf}}
    \subfigure[Random-Polyline Schedule]{
    \includegraphics[width=0.48\linewidth]{figures/25M/random_polyline_72000.pdf}}
    \vspace{-0.1in}
    \caption{\small The examples of long-horizon non-monotonic schedules. The one-power line represents the constant process prediction. \textbf{(a)} The cyclic schedule with 72000 steps, where each half-cycle spans 8000 steps, and the first decay begins after 16000 steps. \textbf{(b)} The random-polyline schedule, consisting of piecewise linear interpolation between randomly selected intermediate learning rates in the range of \( 3 \times 10^{-5} \) to \( 3 \times 10^{-4} \), with LR milestones occurring at intervals of 8000 steps.}
    \label{fig:non-monotonic}
\vspace{-0.15in}
\end{figure}

For general LR schedules, we extrapolate this findings and propose to approximate the total loss reduction term as:
\input{main/derivations/general-rest}

==> main/derivations/general_rest.tex <==
\begin{align*}
    \hatLD(t):= \sum_{k=0}^{t-1}\hatLD_k(t_{k+1})=\sum_{k=0}^{t-1} B (\eta_{k} - \eta_{k+1}) \left(1 - \left(C\eta_{k+1}^{1-\gamma} (t_{k+1}-k)+1\right)^{-\beta}\right).  
\end{align*}
By the definition of $t_{k+1}$~\eqref{eq:tk-Zk}, we have $t_{k+1} - k =\frac{S_{k+1}(t)}{\eta_{k+1}}$. Therefore, we can conclude 
\begin{align} \label{eq:general-loss-reduction}
    \LD(t) \approx \hatLD(t)
    = \sum_{k=1}^{t} B (\eta_{k-1} - \eta_k) \left(1 - (C \eta_k^{-\gamma} S_k(t) + 1)^{-\beta}\right),
\end{align}
where we also change the subscript indices from $k+1$ to $k$. Combining the above ansatz for the loss reduction term with the power-law ansatz for the auxiliary loss in \eqref{eq:auxiliary-loss2} leads to our Multi-Power Law:
\begin{align}
    \cL(t) &\approx L_0 + A \cdot (S_1(t)+S_W)^{-\alpha} - \sum_{k=1}^{t} B (\eta_{k-1} - \eta_k) \left(1 - (C \eta_k^{-\gamma} S_k(t) + 1)^{-\beta}\right).
    \label{equ:MPL}
\end{align}
See~\Cref{app:simp} for the ablation studies on different components of the Multi-Power Law.

==> main/validations/ablation2.tex <==
\subsection{Ablation Experiments}\label{sec:discussion}

We perform ablation studies over key hyper-parameters to assess the applicability and robustness of the Multi-Power Law (MPL). These hyperparameters include the model architectures, model sizes, peak learning rates, batch sizes, and random seeds, incorporating both self-conducted and open-source experimental results.

\paragraph{Model Architectures.} We validate MPL's generalizability across GPT-2~\citep{radford2019language} and OLMo~\citep{groeneveld2024olmo} models to evaluate the generalizability of the MPL across model architectures. 
For GPT-2, we go through the simplified experiments, fitting the MPL on cosine and constant schedules of 24000 steps and predicting the 72000-step loss of the cosine schedule. 
The prediction result is illustrated in \Cref{fig:gpt} and model parameters align to GPT-2 small~\cite{radford2019language}, as detailed in \Cref{tab:model_parameters_summary}.
For the 7B OLMo model, we fit the MPL on the open-source training curve, which employs a linear decay schedule, as shown in \Cref{fig:chinchilla-whole-curve}.
Our results show that the MPL presents a high prediction accuracy across different model types for both self-run and open-source experiments.

\vspace{-1mm}
\paragraph{Model Size}
To test MPL at scale, we train a 1B model on 144B tokens with a batch size of 2M-token and peak LR of $2\times10^{-4}$ for training stability. The model architecture matches Llama-3.2-1B~\citep{dubey2024llama} and is detailed in \Cref{tab:model_parameters_summary}. Simplified experiments involve fitting MPL to 24000-step constant and cosine schedules and predicting the 72000-step loss for both, as shown in \Cref{fig:long-loss-1b-opt-long}. Results demonstrate MPL’s consistent performance across model sizes, as well as the robustness under a different peak LR and batch size.

\vspace{-1mm}
\paragraph{Peak Learning Rate}\label{sec:peak-lr-ablation}
We further investigate MPL’s robustness across varying peak learning rates. While prior experiments fixed the peak learning rate at $3 \times 10^{-4}$, empirical observations of two-stage schedules reveal deviations at higher rates, as illustrated in \Cref{fig:coef-law}. Therefore, we run full experiments with peak learning rates of $4 \times 10^{-4}$ and $6 \times 10^{-4}$ on 25M models, yielding average $R^2$ values of 0.9965 and 0.9940 respectively, underscoring MPL’s consistently decent accuracy while accuracy degrading as peak LR goes up. The training and test set conform to \Cref{tab:set-details} and the fitting results are shown in \Cref{fig:peak-lr-ablation}.

\vspace{-1mm}
\paragraph{Batch Size}
We extend experiments to batch sizes of 64 and 256 sequences on 25M models, complementing the prior 128-sequence (0.5M) results, with sequence length of 4096. MPL maintains high accuracy, with $R^2$ values exceeding 0.9970 across all cases, as illustrated in \Cref{fig:batch-size-ablation}. These experiments indicate that, while the
coefficients of MPL are batch-size dependent, the functional form of MPL remains robust across
varying batch size configurations

\vspace{-1mm}
\paragraph{Random Seeds}
To assess the influence of random seed variability, we train a 25M model over 24000 steps using cosine schedules with three distinct seeds. As shown in \Cref{fig:random-seed}, the loss values exhibit a standard deviation of approximately 0.001, establishing a lower bound for prediction error and highlighting MPL’s precision.
